Lifting The Grey Curtain: A First Look at the Ecosystem of CULPRITWARE

Mobile apps are extensively involved in cyber-crimes. Some apps are malware which compromise users' devices, while some others may lead to privacy leakage. Apart from them, there also exist apps which directly make profit from victims through deceiving, threatening or other criminal actions. We name these apps as CULPRITWARE. They have become emerging threats in recent years. However, the characteristics and the ecosystem of CULPRITWARE remain mysterious. This paper takes the first step towards systematically studying CULPRITWARE and its ecosystem. Specifically, we first characterize CULPRITWARE by categorizing and comparing them with benign apps and malware. The result shows that CULPRITWARE have unique features, e.g., the usage of app generators (25.27%) deviates from that of benign apps (5.08%) and malware (0.43%). Such a discrepancy can be used to distinguish CULPRITWARE from benign apps and malware. Then we understand the structure of the ecosystem by revealing the four participating entities (i.e., developer, agent, operator and reaper) and the workflow. After that, we further reveal the characteristics of the ecosystem by studying the participating entities. Our investigation shows that the majority of CULPRITWARE (at least 52.08%) are propagated through social media rather than the official app markets, and most CULPRITWARE (96%) indirectly rely on the covert fourth-party payment services to transfer the profits. Our findings shed light on the ecosystem, and can facilitate the community and law enforcement authorities to mitigate the threats. We will release the source code of our tools to engage the community.

==> body/bak/005_profile.tex <==
%# -*- coding: utf-8-unix -*-
% !TEX program = latex
% !TEX root = ../sample-sigconf.tex
% !TEX encoding = UTF-8 Unicode


\section{Characterizing \target{}}

% Illegal behaviors are so prevalent that they can be found in every scene. As the manifestation of illegal behavior in the mobile ecosystem, Culpritware also shows a variety of behaviour patterns.
% They serve as the new propagators of fraud, violence and pornography in the Internet century.

% Although they have caused huge economic suffer, the security community don't have enough understand of these apps.
% Before our work, most people even safety practitioners consider them as a whole. 
% However, because of the multiple behaviour patterns of Culpritware, it will omit meaningful features if seemed them as a whole. 
% To better perform our subsequent analysis, we should first classify them to different categories by their behaviour patterns.
% However, there is a lack of specific categorizing rule for Culpritware. To solve this problem, we begin our study from categorizing Culpritware patterns.
In order to have a preliminary understanding of the app-enabled cybercrime, we inspect the Culpritware by imitating the victim. Firstly, we inspect the artifices utilized by perpetrators to understand how victims take steps to the artifices and to get the prevalent of these artifices. Then we inspect how the perpetrators suppress supervision to transfer the illicitly obtained funds. All these above mentioned work is done manually by our team number.

%To ensure the accuracy of the criteria, our team consists of three members of security engineers, and before simulating, our team members have carefully studied the previous reports about crime~\cite{andow2019policylint}, obtain basic judgement ability.

\subsection{Categorize the Culpritware}

The criteria of Culpritware categorization is built upon the combination of the complaints aggregated from victims and the inspections on the Culpritware.
%By following the procedure adopted by Kevin \etal~\cite{roundy2020many},
We use an iterative process to construct and refine criteria for samples, that is {\it (i)} randomly choose a set of 150 apps,
%sampling 150 Culpritware, 
{\it (ii)} perform the run-time simulation independently and read incident report to describe the artifice,  {\it (iii)} discuss to establish consensus and converge on assigning appropriate category names, {\it (iv)} split the remain X apps evenly for each members, {\it (v)} review all apps that fit a category to prevent the trend that the same category has different behaviour patterns. 
In this paper, we use two-level hierarchy of categories to detail the behaviour of the app. In the worst situation, if the app is no longer valid to simulate and the incident report is also missed, we assign the app as ``Unknown''.

For an example, after manually inspect, we find an app behaves like a financial product which pretend to be an formal loan platform with JD.com icon. And after run-time simulation, we record its profit artifices as follow: \begin{quote}\textit{
    ``This app promises to lend users up to 20,000\$ money without interest, but requires users to submit an activation fee of 500\$ first. However, through the victim complaint, after paying the activation fee, the victim didn't get the money they promise.''}
\end{quote}
After establish consensus, we assign the code \textit{Financial} - \textit{Loan Platform} to this app and refine its profit artifices as \textbf{Advanced fee}.


After the procedure, we developed the criteria matrix. The criteria matrix is depicted as Table~\ref{tab:App_category}. The first column of the table is the major category of the Culpritware, the breakdowns of the major category is depicted in the second column of this table. The artifices utilized by perpetrators is depicted in the third column by summarizing the complaints.

As depicted in Table~\ref{tab:App_category}, there are 5 top-categories and 14 sub-categories (\eg, \textit{Financial} - \textit{Loan Platform}) and 13 artifices definitions (e.g., \textit{Advanced Fee}) in reference to the Culpritware 2020-2021 apps.

Taking the matrix, the whole Culpritware set are further tagged by 3 members fully awareness of the criteria. The Figure \ref{fig:classification result} shows the result of our manually assignment of the Culpritware.

\noindent \textbf{Result of the Categoriztion.} Column of 1-2 of Table~\ref{tab:App_category} depict the high diversity of app category, the Culpritware covers a variety of app categories to penetrate the network. The third column of this table reveals the high diversity of artifices, the Culpritware use a variety of artifices to penetrate the life. 

Figure \ref{fig:classification result} shows that financial related Culpritware account for the largest portion, which make up 41.53\% of all Culpritware. Next to the financial is the gambling, which make up 19.81\% of all. And then the sex (9.79\%), service platform (9.78\%) and auxiliary tool (4.30\%).
From the profit tricks, we realize that most of them take advantage of the user's greed, seduce user with high returns and low risk scam.
Especially in the \textit{financial} - \textit{Loan platform}, the largest sub-category (19.81\%), shows the typical high-return scam in cyber crime.


\begin{comment}
To summarize the artifices utilized by perpetrators, we use an iterative process to construct and refine behavior and profit artifices for sample Culpritware.
We introduce the behaviour recorder mentioned in \ref{sec:App_generator} to record the run-time behaviour.

For the first stage, each member randomly choose a set of 150 apps and all members inspect independently.
Each member assigns one or more category codes and the profit artifices description for a specific app.
The code is carefully designed and uses a two-level hierarchy of categories and sub-categories to detail the outstanding behaviour of the app.
For example, the code \textit{Financial} - \textit{Loan Platform} means that the app is closely related to the financial category and exhibits behavior patterns of a loan platform.
And the profit artifices description about this app: \begin{quote}\textit{
    ``This app promises to lend users up to 20,000\$ money without interest, but requires users to submit an activation fee of 500\$ first. However, through the victim complaint, after paying the activation fee, the victim didn't get the money they promise.''}
\end{quote}

If there are no appropriate sub-categories, only top-category code is assigned to the app (\eg, \textit{Financial} - \textit{Unknown}). 
In the worst case, the app is no longer usable when the experiment is conducted and the victim complaint is also missed, we assign the app with top-category \textit{Unknown}.

After independently assigning the first set, we gather all two-level hierarchy categories and profit descriptions, and meet to establish consensus and converge on appropriate category names.
We find that the top-categories in the first round is highly similar, and the major divergence is to distinguish the sub-categories.
After compromise, we set up the initial category of manifestation and reassign the first 150 apps by the entire group. In the meanwhile, we aggregate the initial profit artifices description to each category.

Then the remain xxx apps are split evenly into three parts for engineers. 
We take multiple precautions to prevent bias caused by personal recognize.
Group members will provide explanatory comments about apps, such as ``certain'' or ``uncertain''.
Once group members find an App that not fit into any category, we will take down and decide weather create a new category or modify the exists one.
What's more, all apps that fit a sub-category are reviewed to prevent the trend that the same sub-category has significantly different behaviour patterns. 

After finishing all categorization, we gather apps in the same sub-categories and concise their common profit artifices.
We combine our manual description and the crime report~\cite{andow2019policylint} together, and for some extremely rare cases, we discard these exceptions to prevent cognitive bias from entering them.



\noindent \textbf{Result of Aggregation.}
After all iterations, we summarized an illegal behavior and profit categorization criteria (depicted as Table~\ref{tab:App_category}), with 5 top-categories and 14 sub-categories (\eg, \textit{Financial} - \textit{Loan Platform}) and 13 profit artifices definitions(e.g., \textit{Advanced Fee} in reference to the Culpritware 2020-2021 apps.

First, the numerous behaviour patterns and profit artifices shows that the proliferation of Culpritware, the cyber crime has shown every corner of the network.

What's more, we conclude that Culpritware has a highly organized criminal chain.The victim are often exposed to these apps firstly through advertisement in websites,  auxiliary tool apps or chatting groups(e.g., \textit{Telegram}, \textit{Wechat}). After the victim get the apk, the customer service or region agent will show up and convince the victim to pay money. However, after the victim realise they have been duped, the customer service or region agent has left, even the server of apps will shut down. 
The different perpetrator organizations cooperate with each other and have a clear division of labor, which indicates the Culpritware has formed a set of industrial chain.
%\subsection{Categorize the Culpritware}
%We use an iterative process to construct and refine illegal behavior and profit categories for sample Culpritware.
%For each app, we inspect its behavior for permissions granted, user registration procedures, illegal content usages and payment methods. 
%We first categorized behaviour patterns of apps.
%For the first stage, each member randomly choose a set of 150 apps and all members simulated independently.
% The guidelines were to (1) assign each App with one or more category codes,
%Each member assigns one or more category codes for a specific app.
%The code is carefully designed and uses a two-level hierarchy of categories and sub-categories to detail the outstanding behaviour of the app.
%For example, the code \textit{Financial} - \textit{Loan Platform} means that the app is closely related to the financial category and exhibits behavior patterns of a loan platform.

% and (2) assign codes using a two-level hierarchy of categories and sub-categories that details the outstanding behaviour (e.g., \textit{Financial} - \textit{Loan Platform}). 
%If there are no appropriate sub-categories, only top-category code is assigned to the app (\eg, \textit{Financial} - \textit{Unknown}). 
% However if the App is no longer valid to simulate, we assign the App as ``Unknown'' totally (e.g., \textit{Unknown} - \textit{Unknown}).
%In the worst case the app is no longer usable when the experiment is conducted, we assign the app with top-category \textit{Unknown}.

%After independently assigning the first set, we gathered all two-level hierarchy categories and met to establish consensus and converge on appropriate category names.We found that the top-categories in the first round is highly similar, and the major divergence was to distinguish the sub-categories.
%After compromise, we set up the initial category of manifestation and reassign the first 150 apps by the entire group. 

%The remain xxx apps were split evenly into three parts for engineers. We took multiple precautions to prevent bias caused by personal recognize.
%Group members would provide explanatory comments about apps, such as ``certain'' or ``uncertain''.
%Once group members found an App that not fit into any category, we would take down and decide weather create a new category or modify the exists one.
%What's more, all apps that fit a sub-category were reviewed to prevent the trend that the same %sub-category had significantly different behaviour patterns. 
%\subsection{Study Prevalent of Cyber Crime}
After we conclude the categorizing criteria, we then want to study the prevalent of these artifices in cyber crime. Understanding the distribution of the apps help us to better understand the preference tactics of cyber crime.
We assign all apps with the categorizing criteria, and do an static analysis.

\noindent \textbf{Result of Study.}
%After all iterations, we summarized an illegal behavior and profit categorization table (depicted as Table~\ref{tab:App_category}), with 5 top-categories and 14 sub-categories(\eg, \textit{Financial} - \textit{Loan Platform}, \textit{Sex} - \textit{Pornography trade}).
After assign the categorization criteria on the 565 apps.
we finally got the distribution of the different cyber crime tactics. The Figure \ref{fig:classification result} shows the result of our manually assign.

It's obviously that financial related apps account for the largest proportion, which make up 41.53\% of all Culpritware. Next to the financial is the gambling, which make up 19.81\% of all. And then the sex(9.79\%), service platform(9.78\%) and auxiliary tool(4.30\%).
From the profit tricks, we realise that most of them take advantage of the user's greed, seduce user with high returns and low risk scam.
Especially in the \textit{financial} - \textit{Loan platform}, the largest sub-category (19.81\%), shows the typical high-return scam in cyber crime.

We conclude that the most common tactics in cyber crime is seducing users with scam and the most common behaviour patterns are financial and gambling. 
At the end, we point out that the purpose of Culpritware is to gain illegal profit.

\end{comment}


\begin{figure}
    \centering
    %\vspace{-3ex}
    %\setlength{\belowcaptionskip}{-3ex}
    \caption{Categorization result of 1000 apps in our dataset.}
    \label{fig:classification result}

    \includegraphics[width=.5\textwidth]{figs/prevalent.png}
    \begin{tablenotes}
    \small
    \item[1] Legend shows the top-level categories and for each, the X axis present the second-level categories.
    \end{tablenotes}
\end{figure}



\subsection{Money Laundering in Culpritware}
Inspecting the Culpritware help us understand the tackles of money laundering in the mean time. With the tight scrutinization on illegal transactions, perpetrators migrate the new money laundering tackles into Culpritware. Besides online banking and third-party payment~\cite{yang2019casino}, forth-party payment, money mule and cryptocurrency are leveraged now for money laundering.
To reveal the prevalent of payment services of Culpritware, Our team members sign up an account and initiate payment requests to aggregate the payment process.

Note that it's easy to tell the payment via online banking, third-party payment and cryptocurrency. In order to find money mule payment, we evokes payment request multi-times to observe whether the recipient account changed. If it changed on the fly, we are paying to the money mule. The money mule payment is depicted as Figure~\ref{fig:none-sdk-2}.
Since both the third-party payment and fourth-party payment redirect the payment page to other website~\cite{yang2019casino}, to tell apart the fourth-party payment, we build the collection of licensed third-party payment domain, and any payment page does not fall in this collection is distinguished as fourth-party payment. The fourth-party payment is depicted as Figure~\ref{fig:none-sdk-1}.

\begin{comment}
To the traditional payment services, it's easy to distinguish because they will pull up the formal payment windows and show the payee and transaction amount.
But to , we need additional certification steps.
The Figures~\ref{fig:none-sdk} shows the typical samples of mule based payment services in Culpritware. 

In the fourth-party payment service, if user initial the payment request, the apps will response a transaction website supported by fourth-party services.
From the transaction website, the users can only know that they deliver the money to fourth-party services, but have nothing with where the money goes finally.
Based on this knowledge, our team members record the transaction websites and judge the websites from their UI and payee.
To crowdsourcing payment, they will deliver a single transaction to many different participants.
Each time the user , the server responses a different payee transaction.
To distinguish the crowdsourcing, our team numbers will evokes the payment request with different transaction amount (from small to large) and with different user accounts several times to record the payee information.
If the payee information changes frequently, we seem it as crowdsourcing payment service.
\end{comment}

 \begin{figure}[h]
  \begin{minipage}[t]{1.6in}
   \subfigure[Fourth-party payment service.]{
   \label{fig:none-sdk-1}
   \includegraphics[width=1.3in]{figs/fourthparty.png}}
  \end{minipage}
  \begin{minipage}[t]{1.6in}
   \subfigure[Money mule payment service.]{
   \label{fig:none-sdk-2}
   \includegraphics[width=1.55in]{figs/crowdsourcing.png}}
  \end{minipage}
  \vspace{-0.4cm}
     \caption{Sample of payment services}
     \setlength{\belowcaptionskip}{-3ex}
     \label{fig:none-sdk}
 \end{figure}
%  \vspace{-0.4cm}

\noindent \textbf{Result of the supervision suppression.}
We totally choose 7 different payment services and shows X apps as samples in Table ~\ref{tab:payment}.
Its' obviously that illegal organizations prefer using more covert payment services (\eg, fourth-party and money mule) than traditional payment services, and the online banking payment is the least one used in Culpritware.
And in order to make sure that the payment functions works well, many apps will introduce multiple payment services.


\begin{table}[htb]
\centering
\small
%\setlength{\abovecaptionskip}{-3ex} 
\setlength{\belowcaptionskip}{0ex}
\caption{Payment service analysis.}
\label{tab:payment}
\begin{tabularx}{8.5cm}{lXXXXXXX}
\toprule 
 \textbf{Package Name}\tnote{1} & \textbf{FP} & \textbf{MM} & \textbf{Ali} & \textbf{WX} & \textbf{UP} & \textbf{OB} & \textbf{CC}\\
\hline  
com.jijiehaoqipai.jjhqp & $\bullet$ & - & - & - & - & - & $\bullet$ \\
com.ibxcisekdcas.bieidhs & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & - & - \\
com.game.qebjsa.and & $\bullet$ & $\bullet$ & - & - & $\bullet$ & - & - \\
com.hwgjagwgaw.hwhga & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & - & $\bullet$ \\
com.game.qebr.and & $\bullet$ & $\bullet$ & - & - & $\bullet$ & - & -\\
com.df.bwtnative.op3052 & - & $\bullet$ & - & - & - & - & - \\
com.df.bwtnative.op1014 & - & $\bullet$ & $\bullet$ & - & $\bullet$ & $\bullet$ & - \\
com.qqy.oygj & - & - & $\bullet$ & - & $\bullet$ & - & - \\
com.dawoo.gamebox.sid1338 & $\bullet$ & $\bullet$ & - & - & - & - & $\bullet$ \\
com.adult.zero & - & $\bullet$ & $\bullet$ & - & - & - & - \\
com.tianbo.tbsport & - & $\bullet$ & $\bullet$ & - & - & - & $\bullet$ \\
com.key0.build & - & $\bullet$ & $\bullet$ & - & - & - & $\bullet$ \\
com.android.driver.three651a1 & - & $\bullet$ & $\bullet$ & $\bullet$ & - & - & - \\
com.wj2588.esport & - & $\bullet$ & - & - & - & - & - \\
com.youzu.android.snbx & - & $\bullet$ & - & - & - & - & $\bullet$ \\
meishi.ap & - & $\bullet$ & - & - & - & - & - \\
com.binli.qipai.gp & - & $\bullet$ & $\bullet$ & - & - & - & - \\
com.tea.pincha51 & $\bullet$ & - & - & - & - & - & $\bullet$ \\
\midrule
 \textbf{Total} & \textbf{7} & \textbf{15} & \textbf{9} & \textbf{3} & \textbf{6} & \textbf{1} & \textbf{7}\\
\bottomrule 
\end{tabularx}
\begin{tablenotes}
\footnotesize
\item[1] FP: Fourth-party payment, MM: Money mule, Ali: Alipay, WX: Wechat-Pay, UP: Union-Pay, OB: Online bank, CC: Cryptocurrency
\end{tablenotes}
\end{table}

%According to our manually simulation and judgement on X apps, we form a list of seven common payment services(e.g., fourth-party, crowdsourcing, digital currency) in illicit apps. Our experimental analyses reveal that the Culpritware often leverage the money laundering services to handle transactions, in order to avoid supervision.

%Second, we point out the preference profit patterns of Culpritware. Different from previous studies, we rarely see traditional malware (\eg, \textit{hijack}, \textit{torjan}) in our datasets. In the contrary, our analysis result shows that most Culpritware make profit through deceiving, seducing or menacing devices holders instead of attacking devices. Illegal developers focus more on the financial, gambling or sex themes (totally 71.13\% of all) where they can get profit directly from users. The core of Culpritware is no longer how to hijack the devices, but how to dupe users to gain direct benefits.

%Combined above results, we list the following findings:(1) Culpritware covers a wide range of scenarios, especially in the financial and gambling. (2) Culpritware has formed a set of industrial chain that different illegal organizations cooperate with each other and have a clear division of labor. (3) Most of Culpritware make profit through deceiving, seducing or menacing users rather than attacking devices. The focus of crime has shifted from the device to the device user.

%\vspace{-5ex}



%\subsection{Profit Patterns Study}
%In addition to the illegal behaviour pattern, the profit patterns is also an essential component of behaviour patterns. The rest of this section details the apps' profit patterns and the payment methods.

%\textbf{Profit Patterns.} With simulating all apps, we operate from victim's perspective until finish a complete criminal process.
%We find that some apps will offer a payment entrance to users through different methods (e.g, \textit{membership recharge}, \textit{virtual currency recharge}), but some apps will depend on platform service or other methods.
%It's obviously that different apps have their special patterns to get profit.Unlike the official apps, the Culpritware will leverage illegal profit patterns which act as the core part of illegal behaviours.To understand the profit patterns can complete the investigation of app dynamic behavior patterns.
 
%Combined with some previous studies about crime behaviour\hypo{cite here}, we formulate the profit categories(e.g.,\textit{Service commission}, \textit{advanced fee}).Because of the closely relation between behaviours patterns and profit patterns, we decide to attach the profit patterns as an extra performance item of behaviour patterns.What's more, we find a behaviour pattern will have no less than one profit pattern, and a profit pattern also will appear in different behaviour patterns.After establishing consensus on the group discussion, we set up the 1 to n relation ships between behavior pattern and profit pattern, see in Tab~\ref{tab:App_category}.



%\subsection{Insights from Manual Analysis}
%In this section we present other insights gathered from manual analysis, which form the basis for analysis in later sections.

%\noindent\textbf{App generator usages in Culpritware.}
%\hyf{we still need to rewrite this.}
%While manually categorizing apps,
%we find that illegal apps are rampant not only because of the scope of coverage but also their enormous amount.
%Many inferior quality, counterfeit or unhealthy apps spread widely among people.
%In extremely cases, some websites offer dozens of apk's download links (i.e, ).

%After we check decompiled files, we find many apps developed based on the App generator.
%The App generator provides the boilerplate code\hypo{citation} and H5 interface to the developer, which reduces the threshold of app development and lifts the cross-platform compatibility.
%According to the App generator, developers can create apps rapidly by only provide web based code (HTML, javaScript, CSS and etc.) and resources files.























==> body/bak/006_feature.tex <==

\section{Analyze THE Culpritware}
%In the previous section, we inspect the Culpritware and conclude their categorizing criteria.
%In this section, we further analyze the features of Culpritware.
%Culpritware consists of local resources in the APKs and remote services providing remote resources and functionalities.
% According to the composition characteristics of the app, we divide our research into two part: native apk study and remote services study.

% Unlike some pure stand-alone software, Culpritware serves as the medium between illegal organization and users. The remote servers collect sensitive information and response user request, is an integral part of app.
% To guarantee the persuasion of study, we perform our study from two aspects: local resources analysis and remote service analysis.

\subsection{Research Questions Design}
In the previous section, we inspect the Culpritware and conclude their categorizing criteria.
In this section, we further focus on the features of Culpritware itself. To better distinguish the features in different tactics and find more reliable findings, we perform our analyzing on apps divided by our categorizing criteria to exhibit the difference between them.
And considering the characteristic of hybrid app mentioned in background, we study the Culpritware from three perspective: local apk development, remote services and propagation methods.
Our study is driven by the following research questions:

\noindent\textbf{RQ1: How the Culpritware are developed?} \\
To understand the reason for the proliferation of Culpritware, we conduct analysis on the development procedure of Culpritware.
In particular, we compare the difference between Culpritware and official apps to identify the technique and the special design facilitating Culpritware development.

\noindent\textbf{RQ2: How do Culpritware hide remote services?} \\
Culpritware tends to hide their remote services to evade investigation and regulation.
We conduct analysis on the geographical, registrar and life-cycle features of domain names and IP addresses exposed in Culpritware.
Based on the analysis results, we further demystify how the Culpritware maintainers keep their remote services stealthy.

\noindent\textbf{RQ3: How do Culpritware propagate among target users?}\\
After understanding the proliferation of Culpritware, it is critical to investigate the propagation of Culpritware.
Specifically, we conduct analysis on the target users and how Culpritware propagate amongst these users.

\subsection{Local apk development Analysis}
% In local resource analysis, we perform many perspectives. We've simplified these into three questions about:
% The native APK experiences the process of development, propagation, and finally attaches to the victim app list.
% we summarize our analysis in answering the following two research questions:

%\begin{tcolorbox}[size=title]
%\textbf{RQ1: How the Culpritware are developed?}
%To understand the reason for the proliferation of Culpritware, we conduct analysis on the development procedure of Culpritware.
%In particular, we compare the difference between Culpritware and official apps to identify the technologies and the special features facilitating Culpritware development.
%\end{tcolorbox}
In order to understand the proliferation of Culpritware, the development process of Culpritware is inevitable for us to figure out.
To answer the RQ1, we present our research scheme and results as follows.

\begin{figure}
    \centering
    \includegraphics[width=.45\textwidth]{figs/Appgenetrator-new.png}
    \setlength{\belowcaptionskip}{-3ex}
    \caption{App generator distribution(the ratio of Apps) in the two-level categorization}
    \label{fig:APP Generator}
\end{figure}

\begin{table*}[]\scriptsize
    \centering
    \caption{Third-party library}
\label{tab:Third_party}
\begin{threeparttable}
\begin{tabular}{p{10pt}p{50pt}p{40pt}p{20pt}p{50pt}p{40pt}p{20pt}p{30pt}p{30pt}p{10pt}p{30pt}p{30pt}p{10pt}}
\toprule
%\multirow{2}{*}{Item} &
& \multicolumn{3}{c}{Top 20 Java Library in Culpritware} & \multicolumn{3}{c}{Top 20 Java Library in Benign Apps}
& \multicolumn{3}{c}{Top 20 JavaScript Library in Culpritware} & \multicolumn{3}{c}{Top 20 JavaScript Library in Benign Apps} 
\cr\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
\textbf{Rank} & Name & Category\tnote{1} & Rate\tnote{2} (\%) & Name & Category & Rate(\%) & Name & Category & Rate(\%) & Name & Category & Rate(\%) \cr  
\midrule

\textbf{1} & ZXing & Dev Tool & 47.6 & WXpay & Payment & 66.0 & JQuery & Dom & 13.0 & JQuery & Dom & 33.5\\
\textbf{2} & Glide & Dev Tool & 46.0 & OKHttp & Dev Tool & 65.0 & Platform.js & Dev Tool & 10.8 & Swiper & Res Handle & 29.4\\
\textbf{3} & OKHttp & Dev Tool & 45.3 & Google Gson & Dev Tool & 62.0 & Director & Dev Tool & 5.9 & Vue & Dev Tool & 21.6\\
\textbf{4} & Fastjson & Dev Tool & 39.7 & Alipay & Payment & 49.0 & Filereader.js & Forms & 5.9 & Platform.js & Dev Tool & 18.2\\
\textbf{5} & UniversalImageLoader & Dev Tool & 30.9 & getui & Dev Tool & 45.0 & Request & Utility & 5.9 & Device.js & Touch & 14.6\\
\textbf{6} & Google Gson & Dev Tool & 29.8 & Facebook & Social Network & 41.0 & Vue & Dev Tool & 5.4 & Request & Utility & 13.3\\
\textbf{7} &  Nine Old Androids & Dev Tool & 25.1 & Fastjson & Dev Tool & 38.0 & vConsole & UI & 4.8 & Director & Dev Tool & 12.9\\
\textbf{8} & WXpay & Payment & 24.5 & Glide & Dev Tool & 36.0 & Device.js & Touch & 4.3 & Filereader.js & Forms & 12.9\\
\textbf{9} & DCloud & Dev Tool & 23.5 & Bugly & Analytics & 34.0 & Video.js & Res Handle & 3.8 & Fastclick & Touch & 8.7\\
\textbf{10} & Iflytek Speech & Dev Tool & 18.0 & Xiaomi Push & Dev Tool & 30.0 & ECharts & Utility & 3.2 & Zepto & Dom & 8.5\\
\textbf{11} & Bugly & Analytics & 16.6 & Apache Http & Dev Tool & 27.0 & Swiper & Res Handle & 3.2 & Moment & Utility & 6.6\\
\textbf{12} &  Facebook & Social Network & 16.6 & Umeng Analytics & Analytics & 25.0 & Lodash & Dev Tool & 2.7 & Html2canvas & Res Handle & 5.5\\
\textbf{13} & Alipay & Payment & 16.4 & Bolts & Dev Tool & 23.0 & Moment & Utility & 2.7 & iScroll & Touch & 5.5\\
\textbf{14} & Bolts & Dev Tool & 13.6 & Gtihub & Dev Tool & 20.0 & clipboard & Utility & 2.2 & Ionic & Touch & 2.5\\
\textbf{15} &  Umeng Analytics & Analytics & 13.2 & GMS & Dev Tool & 17.0 & layer & UI & 2.2 & Mobiscroll & Touch & 2.4\\
\textbf{16} & Apache Common & Dev Tool & 12.0 & Alibaba Amap & Map/LBS & 16.0 & Qrcodejs & miscellaneous & 2.2 & Angular.js & Dev Tool & 2.0\\
\textbf{17} & Jiguang & Dev Tool & 11.8 & Umeng Push & Dev Tool & 16.0 & Socket.io & Utility & 2.2 & Cropper & Res Handle & 1.9\\
\textbf{18} &  Baidu Map & Map/LBS & 11.0 & Xinge & Dev Tool & 12.0 & Form & Forms & 1.6 & Axios & Dev Tool & 1.9\\
\textbf{19} & Xiaomi Push & Dev Tool & 9.7 & Baidu Map & Map/LBS & 11.0 & Store.js & Utility & 1.1 & Pdf.js & UI & 1.8\\
\textbf{20} & butterknife & UI & 9.0 & MessagePack & Utility & 10.0 & Angular.js & Dev Tool & 1.1 & Underscore & Dev Tool & 1.3\\
\bottomrule
\end{tabular}
\begin{tablenotes}
\footnotesize
\item[1] 12 categories in total: Dev Tool (Development tool), UI (User interface), Dom (Web DOM tree operation), Forms (Web forms operation), Social Network (Social app library), Analytics (Mobile analytics), Payment (Payment method), Map/LBS (Map or location), Touch (Mobile touch), Res handle (Resource handling such as image, video and audio, etc), Utility (Offer help), Miscellaneous (other libraries).
\item[2] Rate is equal to the number of each labrary divided by the number of apk, witch represent the use frequency of each library in Apps.
\end{tablenotes}
\end{threeparttable}
\end{table*}

\subsubsection{\textbf{App Generators in Culpritware.}}
Mobile apps are increasingly created by app generators nowadays.
To verify the influence of app generator on the development process of Culpritware, we leverage the app generator extractor detailed in Section~\ref{sec:dataset_and_method} to detect app generator based apps.
% to detect the development method of apps. 
% In order to avoid the deviation of different scenarios, we combine the categorization in \textbf{Section~\ref{sec:category}}.

Through 763 apps, we identify 9 different app generators in 260 apps.
We find that the proportion of app generators (34\% of all apps) is extremely high, while the number in official market is even less than 1\%.
To better understand the contribution of app generators, we conclude our analysis result in Figure~\ref{fig:APP Generator}, which shows the statistics of the app generator usages in different categories.
From the result, we find that the apps in top-category \textit{financial} use app generator (53.81\% of all apps) more frequently than the other top-categories.
Even in the least frequently used \textit{gamling} category, there are still 11.12\% of them use app generator.
For all app generators in Culpritware, the most frequently used generators are \verb|DCloud| and \verb|APICloud|, respectively occupying 62.66\% and 24.68\% of all app generators.
Other app generators (\eg, \verb|Appcan|, \verb|apkeditor|) rarely appear.

Based on analysis result above, we can infer that Culpritware extensively utilize app generators to facilitate development.
It also indicates that while the app generator providing convenience to ordinary developers, it also give  opportunities to illegal developers to take advantage of their management oversight.
These app generators need additional regulation to prevent the proliferation of Culpritware.
% It also point out that some official App generators(e.g, \verb|Dcloud|, \verb|APIcloud|, \verb|Bufan|) are lack of regulation, causing the further spread of Culpritware.

\subsubsection{\textbf{Third-Party Libraries in Culpritware.}}
% Besides the App generator, we also
%find that illegal developers highly  rely on third-party libraries,
%especially libraries about the customer service, login registration and others.To 
% study the usage of third-party libraries in Culpritware. 
% In this work, we analyse the decompiled files by \resextractor.
% Considering the difference between App Generator based apps and the native based apps, we detect java libraries of native based apps and JavaScript libraries of App generator based apps respectively.
%What's more, we compare the illegal apps with the corresponding structure benign apps independently to better exhibit.
%Although it's common that developers will leverage third-party libraries to accelerate their development, the frequency and preference of libraries are different.

%We know that JavaScript files are an important component of dynamic web pages, used for data processing and web interaction. 
%Therefore, there are many JavaScript third-party libraries facilitate rapid development by developers.
%So we focused on JavaScript files for analysis and statistics, in order to illustrate certain development characteristics of Culpritware developers.

Besides the App Generator, third-party libraries also play an important role in development process. 
To study the frequency and preference of third-libraries usage in Culpritware, we record all third-party libraries from the local resources.

Considering the bias caused by app generators, we detect Java libraries of non-generator apps and JavaScript (JS) libraries of generator based apps, respectively.
For non-generator apps, we leverage LibRadar~\cite{libradar} to detect Java libraries.
For generator based apps, we introduce an authority JS libraries record website~\cite{Jslib}, which collects well complete JS library information, to detect JS libraries.
According to the previous study~\cite{libradar}, they grouped all libraries into 12 categories (\eg, Development Tools, UI) which also be accepted in this paper.

We finally find 154 different Java libraries and 107 JS libraries from 673 apps.
We then count the frequency and preference and show the top 20 java and JS libraries in Table~\ref{tab:Third_party}.
From the usage rate, it obviously shows that Culpritware uses fewer third-party libraries than official apps, whatever Java or JS libraries. 
Besides the ratio of third-party libraries, the result also shows the preference difference between Culpritware and official apps.
We conclude that official apps use more payment, analytic and utility libraries, while the Culpritware introduce more essential development tools and GUI component libraries to facilitate development.

Combined above results, we indicates that Culpritware uses fewer third-party libraries and prefer to use libraries related to basic development.
It indicate that the Culpritware may contain less functionality than official ones.

% To further understand the difference between each categories of Culpritware, we detect each category of Culpritware respectively.
% In Figure~\ref{fig:APP lib}, we XXXXXX\hypo{HYB rewrite here}
\begin{table}[htb]
%\setlength{\abovecaptionskip}{-3ex} 
\setlength{\belowcaptionskip}{0ex}
\caption{Permission Requirement Analysis.}
\setlength{\belowcaptionskip}{0ex}
\label{tab:permissions}

\begin{threeparttable} 
\begin{tabularx}{8cm}{lXXl}  
\toprule 
 \textbf{Category} & \textbf{Sensitive} & \textbf{insensitive} & \textbf{feature}\\
\midrule  
Sex  & X  & X & X \\ 
Gambling &  X & X & X\\ 
Financial  & X & X & X \\
Service Platform & X & X & X \\
Unknown & X & X & X \\
 \textbf{Benign} & 8.20 & 66.11 & 4.33 \\
\midrule
 \textbf{Total} & \textbf{6.68} & \textbf{23.73} & \textbf{1.24}\\
\bottomrule 
\end{tabularx}
\begin{tablenotes}
\footnotesize
\item[1] The number in the chart represent the average number of each category
\end{tablenotes}
\end{threeparttable}
\end{table}

\subsubsection{\textbf{Application Permission requirement}}
Due to the security design of Android system, apps need to be authorized by the user to obtain sensitive permissions, such as \verb|ACCESS_FINE_LOCATION| and \verb|CAMERA|.
The user permissions requirement indicates the privacy information they can acquire and the system control capability they can access.
To verify the offensive of Culpritware, we analyze the user permission and feature requirements to study the intentions and ability of Culpritware to damage the Android system.

We record all features and permissions from Mainfest.xml and distinguish the sensitive permissions by the Google's statement. 
And to better exhibit our analysis result, we present the results in the table~\ref{tab:permissions}. 
The result shows that the permission and feature requirements of Culpritware are all much lower than those of official apps. The average number of sensitive permissions is only 6.68 in Culpritware, while this number is 8.20 in official apps.
From these low permission requirements, we think Culpritware has low attack maliciousness and ability to damage the Android system. In another word, the Culpritware is not designed for attacking devices, so they lower their feature and permission requirements to pretend that they are not offensive.



%\subsubsection{\textbf{Low Quantity and Quality of Native Resource.}}
%Some previous work \hypo{cite} treat the app quality as app quality, including click delay, page link delay.
%This method perform well to native only apps.
%But when we introduce the H5 page, there is an unavoidable concern about network speed. Since the H5 page will wait for the response of server, it will slower than the page jump implement by native code and cause measurement bias.

%Instead of user experience, we measure the quality of an app by the quantity and quality of its resources.
%The resources are not just the decompiled code, but also the media resource (\textit{MPEG}, \textit{AVI} and etc.) and image resource (\textit{Icon}, \textit{GIF}, \textit{PNG} and etc.). 
%For local resources, we leverage the \resextractor in Section \ref{sec:App_generator} to decompiled the apps.
%For H5 page, we also download all the web resources and combine all types of resources together.By this method, we close the gap between native page and H5 page.

%We finally collect X images, X videos and all developer code from X apps, which represent that each app contains X images and X media resource on average.
%This number indicate that Culpritware owns much fewer media resource than the official apps(contains X images and X media resources on average) which we use everyday.
%What's more, the quality of images and media resources are also poor.The average size of images is only X KB, which means the quality of the image is very low.

%In Section 5.1.3, we have understood the usage of third-party in Culpritware.For code in Culpritware, we divide them into 2 categories: third-party libraries' code and developer's own code.
%In the fast majority of cases, we can find copyright information at the beginning of third-party library files, whether it is a Java third-party library or a JavaScript third-party library.
%So we can use this to distinguish the code of third-party libraries' code from developer's own code.
%We calculate the file size of each categories firstly.We then calculate the percentage of the developer's own code in Culpritware, and find that the ratio is less than 30\%.It is a impressive number which indicates that most of the functionality in Culpritware is implemented by libraries.
%And this is a stark contrast to the official apps, whose developer own code occupy more than 80\%.

%With these scarce, low-quality resources, there is no doubt that the Culpritware is humble and lack of user experience.
%Even some apps is imitation of official software, they also 
%just parodied it, lacking many basic functionality.


\begin{tcolorbox}[size=title]
\textbf{Answer to RQ1:}
The developers of Culpritware use multiple methods to facilitate the development features.
\begin{itemize}[leftmargin=*]
    \item[(1)] The usage of app generators promote the mass production of Culpritware. The 34\% of apps in our dataset are developed using app generators(especially in \textit{Financial} category).
    \item[(2)] Compared with benign apps, Culpritware uses fewer third-party libraries and prefer using libraries of \textit{Development Tool} and \textit{UI Components} for basic development. It indicates the Culpritware contains less functionality than official ones.
    \item[(3)] We also find that the user feature and permission requirement is extremely low in Culpritware. It indicates that the Culpritware has low attack maliciousness and ability to damage the Android system.
\end{itemize}
% First, the usage of app generators leads to the mass production of Culpritware.
% 34\% of apps in our samples are developed using app generators and Culpritware of \textit{Financial} category prefer this method.\\
% Second, the extensive usage of third-party libraries also features the development of Culpritware.
% Compared with benign apps, Culpritware uses more libraries of \textit{Development Tool} and \textit{UI Components} for rapid development.\\
% Finally, we also find that the resources of Culpritware is much fewer than official apps, and the percentage of code added by developers is extremely low(less than X\% on average). \\
% According our study of 656 apps, we point out that
% illegal developers take the App Generator as a new trend. 
% They rapidly produce a plenty of apps (34\% of all Culpritware), especially in the \textit{Financial} category.%, formed a unique ecological phenomenon.
% Besides App Generator, we declare that illegal developers heavily rely on third party libraries.
% Not just in the variety of libraries(e.g, Dev Tool and UI), but also in code percentage of entire project. 
% In our dataset, the percentage of code owned by the developers is fairly low (less than X\% average).
According to these findings, we conclude that illegal developers pursue \textbf{high efficiency, single function, low offensive} to facilitate the development process, which causes the proliferation of Culpritware.
\end{tcolorbox}

% \begin{figure}
%    \centering
%    \includegraphics[width=.4\textwidth]{figs/sample.png}
%    \caption{Need 4 figures here}
    \label{fig:APP lib}
% \end{figure}


\subsection{Remote Service Analysis}
% The remote service play an irreplaceable role in Culpritware.
% In order to expose the characteristics of illegal remote services, 
Because of the characteristic of hybrid app which mentioned in background, Culpritware need to liaise with remote services for managing the requests from client. However, the Culpritware tends to hide their services to evade the investigation and regulation.
In this section, we analyze the features of remote services in Culpritware to answer RQ2.
We present our research and result as follows.

%\begin{tcolorbox}[size=title]
% \textbf{RQ3: What is the network structure of illegal remote services?} \\
%\textbf{RQ2: How do Culpritware hide remote services?} \\
%Culpritware tend to hide their remote services to evade investigation and regulation.
%We conduct analysis on the geographical, registrar and life-cycle features of domain names and IP addresses exposed in Culpritware.
%Based on the analysis results, we further demystify how the Culpritware maintainers keep their remote services stealthy.
% Only domain names or IP addresses is exposed in the app.
% Illegal network structures are different from official ones, which shows more insidious.
% To reveal the basic structure, 
%\end{tcolorbox}

% \begin{tcolorbox}[size=title]
% \textbf{RQ4: What's the domain name and IP address corresponding relationship in time dimension?} The corresponding relationship between domain and IP is complex because their Nonlinear relation and dynamic variability.
% We conduct the corresponding graph with time dimension to figure out the features and variation trend.
% \end{tcolorbox}
% \begin{figure*}[hbtp]
%  \begin{minipage}[t]{3.3in}
 %  \subfigure[Contribution of domain registration geolocation]{
 %  \label{fig:domain_geolocation}
 %  \includegraphics[width = 3in]{figs/Domain_geo.png}}
%  \end{minipage}
 % \begin{minipage}[t]{3.3in}
 %  \subfigure[Contribution of IP resolve geolocation]{
 %  \label{fig:ip_geolocation}
%   \includegraphics[width=3in]{figs/IP_geo.png}}
%  \end{minipage}
 % \vspace{-0.4cm}
  %   \caption{Global Top 15 countries and regions ranked by number of domain registration and IP resolve.}
%     \label{fig:geolocation}
% \end{figure*}

\begin{figure}
    \centering
    \includegraphics[width=.5\textwidth]{figs/Figure 2021-04-18 domain.png}
    \vspace{-4ex}
    \setlength{\belowcaptionskip}{-4ex}
    \caption{Global Top 10 countries and regions ranked by number of domain registration and IP resolve.}
    \label{fig:geolocation}
\end{figure}

\subsubsection{\textbf{Geolocation of Domains and IP addresses.}}

% To identify the country that domains and IP addresses locate, we first query the \verb|whois| information of the recorded domains. 
%To identify the location of domains and IP addresses, we first query the \verb|whois| information of the extracted domains of Culpritware.
% Identifying the geolocation of domains and IP addresses can demystify us of the region where the service is active and the physical place where the server machine locates.
Identifying the geolocation of domains and IP addresses reveals the region of the Culpritware activity and the physical place of the server.
We divide this task into two steps: 1) identify the registered IP address of the domain. 2) locate the IP geolocation of IP addresses.

% To identify the registered IP address of the domain, we first analysis the variety domain information by collecting the \verb|WHOIS| records, and then introduce the knowledge of country-related top-level domain(e.g., \verb|.de| for German) to improve our analysis accuracy.
% Note that we've stored the \verb|whois| information of the extracted domains in Section \ref{sec:Webmonitor}.
%We also introduce the method to locate country based on country-related top-level domain(e.g., .de for German) to improve the accuracy.
% After manually filtering common benign websites, we extracted 2230 domains from a total of 915 apps. which the geo-location information was obtained for 1236 domains. 
%  It's worth noting that most of our Culpritware are collected in China, which can impact on the outcome.
% After our domain geolocation analysis, we show our analysis results in Figure ~\ref{fig:domain_geolocation}.

To identify the registered IP address of the domain, we collect \verb|WHOIS| records of the domains as introduced in Section \ref{sec:Webmonitor}.
We also introduce the knowledge of country-related top-level domain(e.g., \verb|.de| for German) to improve our analysis accuracy.
After filtering benign websites, we collected 1,375 illegal domains from a total of 915 apps.
The result of domain geolocation analysis is depicted in Figure ~\ref{fig:geolocation}~\footnote{It's worth noting that most of our Culpritware samples are collected in China, which can impact on the result.}.
It shows that China and the United States are the largest two countries of Culpritware domains registered. 
There are 743 domains registered in China, far more than any other region or country. % which fits well with the app source composition.

% We first parse out the corresponding IP address, and then analysis the information by querying the \verb|MaxMind|, which reflect the IP geolocation and provide a variety of IP information.
%also checking the geolocation of the IP addresses bounded to the Culpritware domains by querying the \verb|MaxMind| database.  %citation 
To locate the IP geolocation of IP addresses, we first collect IP addresses of domains from DNS services.
Then we query \verb|MaxMind|~\cite{maxmind} database for the IP geolocation information.
We perform our research on 1214 IP addresses collected from 1,375 domains in our Culpritware samples.
The result of geolocation analysis is shown in Figure ~\ref{fig:geolocation}.
%we've obtained the geolocation of 1214 IP addresses from a total of 1892 IP addresses, as shown in Figure~\label{fig:ip_geolocation}. 

% The result are quite different from the domain registered geolocation in Figure ~\ref{fig:domain_geolocation}.
% The IP geolocation result shows that United States ranking first (hosts X IP addresses). % China following, and then a few other countries and regions.
% There are only X\% IP address locate in China, which far less than the domain registration address (X\% in China).

% Combined all above results, we conclude our finding that even our dataset apps mainly active in China(X\% of registered domain locate in China), the illegal organizations prefer to put real server machines in other countries and regions(e.g., the United States, HK) to avoid being tracked.
%However, there are still some similarities that the two highest ranked countries accounting for most of the results.

%The Culpritware samples in our dataset are all from China, yet when locating the domains and IP addresses, the United States takes a large portion of the results. We think it's because the Culpritware developers tend to use proxy severs to hide their identity. 

\begin{table}[htb]
\begin{tabularx}{8cm}{lXl} 
\toprule 
 \textbf{Registrar} & \textbf{Count} & \textbf{Percentage} \\
\midrule  
Alibaba Cloud (Beijing)  & 357  & 24.55\%  \\ 
GoDaddy.com, LLC &  280 & 19.26\% \\ 
Xin Net Technology Corporation & 75 & 5.16\% \\
Alibaba Cloud (WanWang)  & 69 & 4.75\% \\
eName Technology Co.,Ltd. & 50 & 3.44\% \\
NAMECHEAP INC & 50 & 3.44\% \\
MarkMonitor, Inc. & 35 & 2.41\% \\
NameSilo, LLC & 35 & 2.41\% \\
Name.com, Inc & 27 & 1.99\% \\
GANDI SAS & 26 & 1.79\% \\
\midrule
 \textbf{Total} & \textbf{1004} & \textbf{69.05\%} \\
\bottomrule 
\end{tabularx}
\setlength{\belowcaptionskip}{0ex}
\caption{Registrars of Domain.}
 \label{tab:Registrar}
\end{table}


\subsubsection{\textbf{Registrar of Domains.}}
We also analysis the registrar information from the collection of \verb|WHOIS| record, because the registrar information of domains might be directly connected with developers. 
By registrar analysis, we collect 160 different registrars  from 1,375 domains at all.
%get the result of 1375 domains in total, including 160 different registrars.  
The result shows that most of the domain registrars are not developers or their companies, but domain service agents such as \verb|Godaddy|,  \verb|Alibaba Cloud| and etc.
The registrars that contain more than 5 domains are listed in the Table ~\ref{tab:Registrar} and these companies are all domain service agents. 
The number of domains hosted by these above-mentioned agents amount to 1180, which represents 85\% of all extracted domains.

%The result of registrar information shows that the illegal organizations tend to use domain service agents and proxy severs to register the domains in order to hide their real identity.


\subsubsection{\textbf{Life-cycle Assessment.}}
The life-cycle is also an important feature of illegal domain, which indicates the duration of crime.
If the remote server has been closed, the request will be missed or receive the response with an error status code such as \textit{404, 500} and etc.
To analysis the life-cycle of the illegal domain, we observe the response content of remote services.
What's more, to ensure that the request packet we construct conforms to the rules, we launch the apps on the real phones to send the requests to the server.
Leverage the large pool of phones, which consist of X phones, we have the capability to monitor the survival status of X Culpritware.
%Based on the knowledge that internet apps will liaise with remote server while launching, requiring resource, sending commands and etc.
%So if an app is dead, the remote server has been closed, the apps will receive the response with an error status code such as \textit{404, 500} and etc.
For automatic observation, we first leverage the Android assistive tools to automatically install the apk to Google Pixel 3 and then launch the app up.
In the meanwhile, we initiate a subprocess to capture network packets during the launching with the assistance of mitmproxy.
We also filter out some unwanted packets, such as \verb|Umeng| and \verb|Google service|. 

After collecting the survival information, we also need to know the start time in order to calculate the Life-cycle.
But it's hard to obtain the accurate begin time of domain usage, so we take the last modification time of \textit{AndroidManifest.xml} file as the start time of app release, also as the valid time of the illegal domains.

After X days of continuous monitoring of X Culpritwares, we acquire the life-cycle result and show in Figure X.
It illustrates an obvious phenomenon that the illegal domain just survival a short period of time on the whole.
The average survival time is X days and only X\% of apps' domains survival more than X days. From the perspective of different Culpritware categories, we can find that the life-cycle of financial products is shortest (X days on the average) and the sex apps is longest (X days on the average).

\begin{figure}
    \centering
    \includegraphics[width=.4\textwidth]{figs/Appgenetrator-new.png}
    \setlength{\belowcaptionskip}{2ex}
    \vspace{-3ex}
    \caption{Sample}
    \label{fig:life cycle}
\end{figure}

%\begin{tcolorbox}[size=title]
%\textbf{Answer to RQ2(1):}
%According to our continuous monitoring and analysis, we conclude the basic %structure features of remote services to hide themselves:
% After our continuous monitoring, we point out the phenomenon that illegal developers prefer to locate their server in other countries to avoid tracing. 
% In this paper, almost all of Culpritware came from China, but the geolocation result shows the remote servers locate in many other countries, especially in US(X\%) and HK(X\%).
% What's more, most registrar of domain are domain service agents(e.g, Godaddy, Alibaba), which completely hiding the real registrant information.

% Most notably, after X days surveillance monitoring, we have summarized the life cycle of Culpritware.  
% Most of Culpritware(X\%) will dead within X days after been developed.
% It's a significant finding that, unlike official software, Culpritware has a extremely short life cycle, which makes it more secretive.

%\begin{itemize}[leftmargin=*]
%    \item[(1)] Even our dataset apps mainly active in China(X\% of registered domain locate in China), the illegal organizations prefer to put real server machines in other countries and regions(e.g., the United States, HK).
    %Culpritware samples in our dataset mostly collected from China, but the geolocation results show the remote servers locate in many other countries, especially in US(X\%) and HK(X\%). What's more, Culpritware developers commonly buy domains from domain service agents(e.g, Godaddy and Alibaba). The real registrant information remains hidden.
%    \item[(2)] Illegal organizations tend to use domain service agents and proxy severs to register the domains.
%    \item[(3)] The life cycle of remote services is very short. Most of domains in Culpritware(X\%) will dead within X days after been released. 
%\end{itemize}
%\end{tcolorbox}

\subsubsection{\textbf{The corresponding relationship between Domain and IP}}

To conduct the corresponding graph with time dimension, we first leverage the \verb|DNS| technique to find out the corresponding relationship.
However, because the relationship will change over time, we then record the relationship collected from \verb|DNS| and dynamic update the relationship every day.
We continuously collected the \verb|DNS| information from February 1, 2021 to May 1, 2021 on 2230 domains, and finally obtained 1892 IP addresses during the period. 

While monitoring, We find an abnormal phenomenon that illegal domains will frequently change their corresponding IP addresses.
\begin{figure}
    \centering
    \includegraphics[width=.4\textwidth]{figs/ip_day.png}
    \setlength{\belowcaptionskip}{2ex}
    \vspace{-3ex}
    \caption{Domain-IP corresponding changing sample}
    \label{fig:ip day}
\end{figure}
%In order to expose this phenomenon, we keep monitoring daily and record the change of the IP addresses bind to the domains from our dataset. 
The monitoring records shows that X\% of domains have changed the binding IP addresses for at least once in two months.
The least time between domain and IP corresponding is even less than 1 day, and the average days of all domains and IP addresses corresponding change is only 16.94 days, which means that the relationship is extremely mutable.

\begin{figure*}
    \centering
    \includegraphics[width=.9\textwidth]{figs/IP-domain relationship.png}
    \setlength{\belowcaptionskip}{2ex}
    \vspace{-3ex}
    \caption{Domain-IP corresponding changing sample}
    \label{fig:domain relationship}
\end{figure*}

To further exhibit the complex corresponding relationship, we also show an example in Figure~\ref{fig:domain relationship} to demystify the unusual phenomenon.
We conclude three unusual phenomenon in the corresponding relationship:
{\it (i)} The different domains extracted from different apps will map to the same IP address at a certain time, e.g., the domain yg19.top( from \textit{w2a.W2Awww.yg19.top}) and yuereee.top( from \textit{w2a.W2Awww.yuereee.top}) have different IP address before, but map to the IP 47.74.14.254 from May 18, 2021 until the server is down.
{\it (ii)} There exists super servers where many domains corresponding to and behave stably, e.g., the IP 184.168.13.241 has up to 15 different domain point to at the same time( due to space constraints, only four domains are shown). Through our monitoring, there corresponding relationship are very stable and never changed until May 1, 2021.
{\it (iii)} What's more, the domains will map to the IP addresses which used by other domains before, such as uk919.com( from \textit{com.lckctasu}) corresponding to the IP 157.240.20.18 at April 20, 2021, which used by facai1788.com( from \textit{com.hw.app1127}) before.
%Our approach is to find out the mapping relationship between different domains and IP addresses, and we generated a graph of the relationship between domains and IP addresses. 

%To better exhibit our finding, we select a part of our record and plot it in Figure X. 
%From Figure x, there are many different domains and IP addresses that are related to each other. 
These relationship are so complex and mutable. Their relationship even beyond the bounds of different category, which become a very special ecological scene for illegal domains.

% As an example, we find an IP address(\textit{34.102.136.180}) bound to 34 domains extracted from different apps. By checking the \verb|whois| information of these domains, we found that the registrars of these domains are all GoDaddy.com and the sever of these domains are all whois.godaddy.com. This example prove our idea that different domains bound to the same IP address beacuse of the use of domain service agents.

\begin{tcolorbox}[size=title]
\textbf{Answer to RQ2:}
According to our continuous monitoring and analysis, we conclude the features of remote services to hide themselves:

\begin{itemize}[leftmargin=*]
    \item[(1)] Even the apps in our dataset mainly active in China, the illegal organizations prefer to locate physical server in other countries and regions(e.g., the United States, HK).
    \item[(2)] Illegal organizations tend to use domain service agents and proxy severs to register the domain.
    \item[(3)] The valid period of illegal services is transitory. Most of domains in Culpritware(X\%) will dead within X days after been released. 
    \item[(4)] Illegal ones tend to change the corresponding relationships between IP address and domains frequently. 
    The average days of relationship change are only 16.94 days. 
    More impressed, the domains extracted from different apps will point to the same IP address.
\end{itemize}
%The reason is the widespread use of domain sevice agent by developers.
\end{tcolorbox}



\subsection{Propagation Analysis}
After analyzing the local and remote features of Culpritware, we further focus on the propagation process and the target users of the Culpritware.
We present our study from the design of Culpritware registration and invitation to answer the RQ3.
%\begin{tcolorbox}[size=title]
%\textbf{RQ4: How do Culpritware propagate among target users?}
%After understanding the proliferation of Culpritware, it is critical to investigate the propagation of Culpritware.
%Specifically, we conduct analysis on the target users and how Culpritware propagate amongst these users.
% \textbf{RQ2: What kind of users are targeted by Culpritware and how they propagate?}
% Considering to better understand the proliferation of Culpritware, it's interesting to investigate the vulnerable groups and the propagation process.
% Finding out the target groups and the propagation can lead to better prevent spread of Culpritware.
%\end{tcolorbox}

\subsubsection{\textbf{User Registration and User Agreements.}}
% When we attempt to answer \textbf{RQ2}, we give up gathering information from audiences devices because of ethic concern.
% Instead, we observe the design of registration and referrer to solve the problem.
% From the developers' perspective, their design of app rest with customers they serve.
% Generally speaking, official apps require the phone number or other platform authorization (e.g, Tecent QQ, Wechat) to sign up a new account, because they are designed for official users. 
% During official registration, the user's privacy protection and security protocol will be given to ensure the user's privacy will not be abused.

To understand the target users of Culpritware, we first focus on how users register.
For benign apps, the registration procedure is straight forward.
An user first provide identification information (i.e. phone numbers, social platform accounts, etc.) to sign up a new account.
Then the app presents a user agreement about usage and privacy policies for user.

Culpritware exhibits abnormal patterns of the registration procedure.
First, many Culpritware require an ``access code'' or ``invitation code'' as a prerequisite for the registration.
% For some of them, this access code is the only entrance.
These codes can be obtained from other registered users of the same app or from specific agents.
Second, the absence of user agreements is common for Culpritware.
User agreements involve a number of corporate obligations and legal guarantees to protect user privacy.
The absence of user agreements means that the users of Culpritware may lack the basic legal and safety awareness.

% But when we observe Culpritware, we find their registration design are abnormal.
% For example, we found that the ``access code'' is mandatory for registration in some apps.
% Some of them even only exhibit a login screen and require an ``access code'' after loading.
% For this type of dissemination, the developer also don't follow security protocols.
% The absence of security protocols is common, we also find other registrations don't show security protocols, or give inaccessible protocols.
% We leverage the manually simulation in Section \ref{sec:dataset_and_method} to statistic the registration methods in Culpritware.

\begin{table}[htb]
\centering
%\setlength{\abovecaptionskip}{-3ex} 
\setlength{\belowcaptionskip}{0ex}
\caption{Registration and security protocol analysis.}
\label{tab:invite}
\small
\begin{tabularx}{8cm}{lXXl}  
\toprule 
 \textbf{Category} & \textbf{Alive} & \textbf{Invitation} & \textbf{Agreement Absence}\\
\midrule  
Sex  & 33  & 21(63.64\%) & 26(78.79\%) \\ 
Gambling &  73 & 17(23.29\%) & 51(59.86\%)\\ 
Financial  & 56 & 21(37.5\%) & 31(55.36\%) \\
Service Platform & 43 & 2(4.65\%) & 20(46.51\%) \\
Unknown & 31 & 18(56.04\%) & 25(80.65\%) \\
 \textbf{Benign} & 100 & 0(0.00\%) & 4(4.00\%) \\
\midrule
 \textbf{Total} & \textbf{236} & \textbf{79(33.47\%)} & \textbf{153(64.83\%)}\\
\bottomrule 
\end{tabularx}
\end{table}

% Table \ref{tab:invite} shows the difference between benign apps and Culpritware in registration methods.
% The invitation registration method occupy 33.47\% of all Culpritware, while no official app in this way.
From analysis, we summarize the difference of registration procedure of official apps and Culpritware in Table~\ref{tab:invite}.
There are 33.47\% of all Culpritware samples requiring invitation to register.
Especially in \textit{Sex} top-category, the invitation rate is extremely high (63.64\%). 
With further analysis, we find that 81.8\% apps of \textit{Sex} - \textit{Prostitution Transaction Platform} need ``access code'' when registration. 
But the ratio in \textit{Financial} - \textit{Loaning Platform} is only 6.2\%.
We correlate the ``access code" rate to the different cost of illegal activities.
Illegal activities with lower costs tend to attract more users with low registration requirements.
Conversely, high-cost illegal activities like sexual transaction prefer to spread through acquaintances.
It helps for organizers of these risky illegal activities to stay hidden from regulation and investigation.
% We infer this difference is caused by different cost of illegal behaviours.
% If the cost of illegal behaviour is low and easy to escape, the illegal organizations will attract more victims to earn more profit.
% But some high cost behaviours(e.g, prostitution transaction) will reveal their real identity. 
% To ensure users won't report them, illegal organizations prefer to spread through acquaintances, so they use invitation to prevent other unfamiliar users.

At the same time, the absence of user agreement is very common.
Since 64.83\% of all apps haven't a valid user agreement, we conclude that Culpritware targets to specific groups of people, who lack the basic legal and safety awareness.
The gullible crowd will ignore the role of user agreement and mistakenly believe the Culpritware are trustworthy.


\subsubsection{\textbf{Acquaintance Based Propagation.}}
Inspired by the way of registration, we conduct further analysis on propagation methods of Culpritware.
Besides downloading from the market or web advertisements, we also find they spread through acquaintances.

In previous subsection, we find that ``access code" is shared by old users. 
But we don't know clearly about the motivation of old users to share ``access code".
To explain this question, we communicate with customer services and manually simulated the process of promotion.
But due to illegal apps' extremely high vigilance, we  can only contact few part of the customer services.
Most of them refuse to reply our questions.
However, we still find the sharing function in X apps.
There are two ways for users to participate in the distribution process, sharing ``access code" with acquaintances or joining as an agent.
Culpritware rewards the distributors for their propagation contribution.
They may even reward small amounts of cash before harming individuals.

Illegal organizations also allow the user become the agent, the person in charge of the Culpritware operation in a small area.
This kind of hierarchy makes it more difficult to distinguish between the victim and the abuser.

The existence of agents supplements the vacancy in the illegal organizations, making illegal activities more permeable and harder to track.
However, this way of propagation makes the aggregation of app obviously.
Inspired by the Creepware~\cite{roundy2020many} and Polonium~\cite{Polonium}, we conclude Culpritware principle of \textbf{guilt by association (GBA)}:\textit{ illegal activity apps are disproportionately installed on the same intersect groups}.
By disproportionately, we mean in the relation to the likelihood these groups co-install with other groups.

\begin{tcolorbox}[size=title]
\textbf{Answer to RQ3:}
Unlike official apps, we find that Culpritware are designed for specific user groups with exclusivity and low safety sense.
We explore 236 Culpritware apps and record their registration process. The result shows 33.47\% of Culpritware need ``access code" and 64.83\% without valid user agreement.
After analyzing the propagation process, we conclude the \textbf{guilt by association(GBA)} principle applies to Culpritware.

From above work, we conclude that vulnerable groups lack of safety knowledge generally, trust in acquaintances' recommendations or unwary of apk downloaded from unknown sources.

\end{tcolorbox}


==> body/bak/007_developer.tex <==
\section{Profile the Developer behind Culpritware.}
In the previous sections, we have done a comprehensive study on the Culpritware. In the study process, we find that some apps have similar characteristics, which indicates the developers behind them are the same.

To demystify these phenomenon, we take two apps in \textit{Sex} - \textit{Live Porn} category (\textit{com.f8456898990.jvf} and \textit{com.w1217898990.osg}) as the example. 
We first install them on the Pixel 3 to inspect and find they show the similar initial pages which make no difference to the naked eye. What's more, after collecting their URL list, we find their URLs are 81\% duplicated.
We then analysis their developer signatures. Although the MD5 of their developer signatures are different, there still exist some same fields (e.g., \textit{Country}, \textit{email address}).
From all findings above, we claim they belong to the same developer.

In this section, we purpose to profile the developer behind the Culpritware.
To achieve this purpose, we first leverage signature extractor in Sec~\ref{sec:App_generator} to check the validity of developer signatures and collect the basic information.
Combined the findings above, we then propose a developer correlation process with multiple attributions, including developer signature, service domain and snapshots, to gather the apps with highly similarity that reveal the developer constitute behind the Culpritware. 
Finally, we do provenance study to find out apps developed by same developer through Android app collections.


\subsection{Developer Signature Validity Check}
To collect the basic information from Culpritware, we first do the validity check of developer signature collected by the signature collector mentioned in  \textbf{Section~\ref{sec:App_generator}}. 
First of all, we sort out the quote certificates, such as AOSP official certificate, Android tester certificate and app generator certificate.
These certificates are issued by other organizations and have nothing to do with real developers.
We check 654 Culpritware signatures, and find 18.98\% apps using quote certificates(7.9\% AOSP official certificates, 1.6\% Android debug certificates, 9.5\% App generator certificates).

Then we do statistic the omission rate to each fields of signature. 
The result shows that the average omission rate of all fields is 14.98\%, and the omission rate of signatures with missing fields is 24.85\%. 
The most common missing field is \textit{State} and \textit{Country}, which result in 86.16\% incomplete certificates. 
What's more, we introduce the formatting rules. For an example, the \textit{Country} filed should be filled with national abbreviations or area code.
After reviewing, we find X\% of Culpritware signatures violate the formatting rules.

The above findings illustrate that Culpritware signatures have a high percentage of omission and confusion. There are totally X\% apps using non-standard certificates, including quote certificates, omission fields and meaningless fields. 
Therefore, the signatures can't represent the truly identities of developers.
But because of their plenty textual information, they can be used to represent the developer characteristics as an important attribution.  

\renewcommand{\algorithmicensure}{\textbf{Output:}} % Use Output in the format of Algorithm
\begin{algorithm}[h]
  \caption{Developer Association Process} % 名称
  \begin{algorithmic}[1]
    \Require
      $x_0$: initial seed app;
      $I$: iteration number;
      
      $I_{max}$: maximum iteration number;
    \Ensure
       apps collection within $I_{max}$ iterations;
       \State Initial $seed$ with $x_0$, $I_0$ = 0
       \State Initial developer signature, URL domain and snapshots from $seed$;
       \While {$I <= I_{max}$}
        \State extension $x$ += \textbf{Signature Association}\ding{182} apps;
        \State extension $x$ += \textbf{URL Domain Association}\ding{183} apps;
        \State extension $x$ += \textbf{Snapshot Association}\ding{184} apps;
        \State set $I_x$ = $I$
         \For{$x_i$ in $x$ }
      \State set $x_i$ as the new $seed$, $I_i$=$I_x$+1
      \State goto step 2
     \EndFor
    \EndWhile
  \end{algorithmic}
  \label{alg:cluster}
\end{algorithm}

\subsection{Developer constitute Study}
After previous signature validity check, we learn that it's not enough to identify the developer only through their signatures.
And different from previous work~\cite{sebastian2020towards}, which leverage official market registration record, Culpritware spread by unofficial methods without records rather than official market channel.
And Some previous work used code based similarity matching to gather  apps~\cite{zhou2012detecting}. But through previous findings in this paper, we realise that app generator based apps will reuse boilerplate code, cause code based detection performs poorly.

Instead, we leverage the findings in previous sections that remote services domain represent the identity of the developer, such as payment websites and server domain name.
Since changing these things will significantly increase the cost of development.
So we introduce URL similarity in our relevance process. 
What's more, through some previous research, we decide introduce visual similarity concept using apps snapshots collection by snapshot collector mentioned in Sec~\ref{sec:App_generator}.
Finally, we conclude the key attributions to represent the developer characteristic: (1)  \textbf{developer signature certificate} , (2) \textbf{URL domain list}, (3) \textbf{snapshots}.

We present the Workflow ~\ref{alg:cluster} to gather all apps with similar characteristics.
Because different attributions are consist of different types, we design methods for each attribution.

(1) \textbf{Signature Association}\ding{182}: the signature certificate attribution is consist of multiple string fields. 
First of all, we eliminate all quote certificates to avoid bias in association process.
Then we compare remain certificates through all fields. If their filed contents are the same, we call this filed as ``\verb|agreement point|''. 
Among all fields, some have strong correlation property (\textit{certMD5}), while some haven't (e.g, \textit{tate}, \textit{countryName}).
when the strong correlation fields become the ``\verb|agreement point|'', we gather them undoubtedly.
Else, if the strong correlation fields are different, but the ``\verb|agreement point|'' occupy more than half of all fields.
We think these two certificates are highly similar, and also gather them.

(2) \textbf{URL Domain Association}\ding{183}: the URL list attribution is consist of URL domains and IP addresses mentioned in section \ref{sec:Webmonitor}. To improve the accuracy, we also filter out all the Alexa top authority websites. Finally, we compare two URL lists and correlate them if the overlap part is beyond both half of them. 

(3) \textbf{Snapshot Association}\ding{184}: the snapshot attribution is consist of snapshot record in section \ref{fig:workflow}. We leverage SIFT algorithm~\cite{lowe2004distinctive} to get keypoint of a snapshot and use Euclidean distance to get the similarity of images. In order to improve the efficiency of picture comparison, we store the intermediate results of image instead of the raw image.
To determine the boundary, where two images are similar or not, we manually choose some similar images as test dataset.

Theoretically speaking, the attribution extension process can iterate infinitely until all the children nodes can't find any new node. 
However, because of concept deviation, too many iterations will lead to invalid association and data explosion. 
To avoid this situation, we set the max iteration number to 2. By this approach,  we can avoid the association distortion caused by information explosion.

\begin{figure}
    \centering
    \includegraphics[width=.4\textwidth]{figs/cluster3.png}
    \caption{Clustering Result}
    \vspace{-3ex}
    \label{fig:Cluster result}
\end{figure}

The Figure \ref{fig:Cluster result} shows the result of our process, which present the developer consistency in Culpritware. 
In the association graph, there are some clusters don't have any out degree, but the apps in the clusters connect tightly. 
This situation illustrates our association process are very precise. We can gather apps with same developer while not introduce other low similarity apps.

We conclude there exists illegal developer who specialize in developing Culpritware, the biggest cluster owns 7.95\% Culpritware of all, then the second owns 6.69\%.
They have highly URL domain and visual similarity, and most of them are categorized into gambling and financial.
Besides the huge cluster, most of apps can gathered together after our process, only 31.66\% of them can't associate any other app. It indicates that the developers behind the apps will create no less than one apps, even cross different categories, and these developers are organized, not purely individual performance. The association process not only show the relationship between developers and applications, but also can be used to detect Culpritware.

\subsection{Attribution of Developer}
After doing above relevant process, we've gathered bunches of Culpritware with the same developer. However, the number of our dataset is limited, we further want to provenance the developer through other much larger Android app collections to collect more information.
To collect more apps, we leverage Android App collections (e.g, \textit{Koodous}~\cite{koodous}, \textit{Xinyuan}~\cite{xingyuan}) to expand our dataset.
These collections provide different query interfaces, so we parse some common attributes, such as \textit{MD5 Checksum of Certification}, \textit{Organization},
\textit{Email-Address} and etc.

We query different app collections and  record the response messages.
In our research work, we find that the average number of apps correlated by app collections is 3.86.
We also leverage the information collected from the related apps.
After gathering all characters, we then use the cyberspace search engine (ZoomEye~\cite{ZoomEye}, BinaryEdge~\cite{BinaryEdge}) to search more interesting findings. At the meanwhile, we also leverage the user community to search more relevant information about the developer.
To better illustrate our provenance process, we set the Sex-live Porn app \textit{com.w1217898990.osg} as the example.

\begin{figure}
    \centering
    \includegraphics[width=.45\textwidth]{figs/provenance.png}
    \caption{Attribution assessment sample}
    \vspace{-3ex}
    \label{fig:provenance}
\end{figure}

In Figure~\ref{fig:provenance}, we start from \textit{com.w1217898990.osg} and collect its attributions( e.g., URL domain, email address and certMD5). We collect two email address, the signature certMD5 and an already dead URL domain.
We first query the certMD5 and email addresses through Koodous. The result shows that the certMD5 and address-one can't find any related app while address-two associate many other cyber-crime app.
But leverage the google research, we find the valid social account bound with the email-one. We then search the social account on Zoom Eye, and finally got the organization name, it's interesting that the Culpritware developer used be an official app developer organization.

At the meantime, we also record the apps queried from Koodous, and find out an alive domain which used the same IP address as the original dead URL domain, which provides opportunities for dynamic analysis.
What's more, we search the user community such as internet forum and social media, find that some victims complain their suffer and reveal some personal information about the developer.

From provenance, we conclude that some developers not only make Culpritware for cyber-crime, but also make official apps. And using the provenance process, we can find more related information about the illegal developer.
However, due to the complexity and variability of the information, it is hard for us to summarize a set of completely automated search methods. 


==> tables/javajs.tex <==
\begin{sidewaystable*}[t]
\scriptsize
\centering
\caption{Summarization of Third-Party Libraries in App Samples}
\label{tab:Third_party}
\begin{threeparttable}
% \begin{tabular}{p{10pt}p{50pt}p{40pt}p{20pt}p{50pt}p{40pt}p{20pt}p{30pt}p{30pt}p{10pt}p{30pt}p{30pt}p{10pt}}
\begin{tabular}{ccccccccccccc}
\toprule
%\multirow{2}{*}{Item} &
& \multicolumn{3}{c}{Top 20 Java Library in \target{}} & \multicolumn{3}{c}{Top 20 Java Library in \normal{} Apps}
& \multicolumn{3}{c}{Top 20 JavaScript Library in \target{}} & \multicolumn{3}{c}{Top 20 JavaScript Library in \normal{} Apps} 
\cr\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
\textbf{Rank} & Name & Category\tnote{1} & Rate\tnote{2} (\%) & Name & Category & Rate(\%) & Name & Category & Rate(\%) & Name & Category & Rate(\%) \cr  
\midrule

\textbf{1} & ZXing & Dev Tool & 47.6 & WXpay & Payment & 66.0 & JQuery & Dom & 11.9 & JQuery & Dom & 52.3\\
\textbf{2} & Glide & Dev Tool & 46.0 & OKHttp & Dev Tool & 65.0 & Page.js & Dev Tool & 6.8 & Device.js & Touch & 21.4\\
\textbf{3} & OKHttp & Dev Tool & 45.3 & Google Gson & Dev Tool & 62.0 & Vue & Dev Tool & 3.8 & Platform.js & Dev Tool & 19.4\\
\textbf{4} & Fastjson & Dev Tool & 39.7 & Alipay & Payment & 49.0 & Swiper & Res Handle & 3.8 & Request & Utility & 16.1\\
\textbf{5} & UniversalImageLoader & Dev Tool & 30.9 & getui & Dev Tool & 45.0 & Zepto & Dom & 3.2 & Director & Dev Tool & 15.6\\
\textbf{6} & Google Gson & Dev Tool & 29.8 & Facebook & Social Network & 41.0 & Request & Utility & 2.0 & Filereader.js & Forms & 15.5\\
\textbf{7} &  Nine Old Androids & Dev Tool & 25.1 & Fastjson & Dev Tool & 38.0 & Axios & Dev Tool & 1.8 & Angular.js & Dev Tool & 7.0\\
\textbf{8} & WXpay & Payment & 24.5 & Glide & Dev Tool & 36.0 & iScroll & Touch & 1.8 & Fastclick & Touch & 6.7\\
\textbf{9} & DCloud & Dev Tool & 23.5 & Bugly & Analytics & 34.0 & Imagesloaded & Res Handle & 1.6 & Ionic & Touch & 6.0\\
\textbf{10} & Iflytek Speech & Dev Tool & 18.0 & Xiaomi Push & Dev Tool & 30.0 & Platform.js & Dev Tool & 1.6 & Underscore & Dev Tool & 5.9\\
\textbf{11} & Bugly & Analytics & 16.6 & Apache Http & Dev Tool & 27.0 & Grunt & Dev Tool & 1.6 & Date & Utility & 4.9\\
\textbf{12} &  Facebook & Social Network & 16.6 & Umeng Analytics & Analytics & 25.0 & Poly & Utility & 1.6 & iScroll & Touch & 4.5\\
\textbf{13} & Alipay & Payment & 16.4 & Bolts & Dev Tool & 23.0 & Store & Utility & 1.6 & Form & Forms & 4.2\\
\textbf{14} & Bolts & Dev Tool & 13.6 & Gtihub & Dev Tool & 20.0 & Pure & Dev Tool & 1.5 & Moment & Utility & 4.1\\
\textbf{15} &  Umeng Analytics & Analytics & 13.2 & GMS & Dev Tool & 17.0 & Html & Dom & 1.5 & Video.js & Res Handle & 4.0\\
\textbf{16} & Apache Common & Dev Tool & 12.0 & Alibaba Amap & Map/LBS & 16.0 & Soc.js & Res Handle & 1.5 & Zip.js & Utility & 3.5\\
\textbf{17} & Jiguang & Dev Tool & 11.8 & Umeng Push & Dev Tool & 16.0 & Fastclick & Touch & 1.3 & Lodash & Dev Tool & 3.3\\
\textbf{18} &  Baidu Map & Map/LBS & 11.0 & Xinge & Dev Tool & 12.0 & Magic & Res Handle & 1.1 & Audio.js & Res Handle & 3.2\\
\textbf{19} & Xiaomi Push & Dev Tool & 9.7 & Baidu Map & Map/LBS & 11.0 & Script.js & Dev Tool & 1.1 & Jasmine & Dev Tool & 2.9\\
\textbf{20} & butterknife & UI & 9.0 & MessagePack & Utility & 10.0 & Director & Dev Tool & 0.9 & Script.js & Dev Tool & 2.8\\
\bottomrule
\end{tabular}
\begin{tablenotes}
\footnotesize
\item[1] 12 categories in total: Dev Tool (Development tool), UI (User interface), Dom (Web DOM tree operation), Forms (Web forms operation), Social Network (Social app library), Analytics (Mobile analytics), Payment (Payment method), Map/LBS (Map or location), Touch (Mobile touch), Res handle (Resource handling such as image, video and audio, etc), Utility (Offer help), Miscellaneous (other libraries).
\item[2] Rate is equal to the number of each labrary divided by the number of apk, witch represent the use frequency of each library in Apps.
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable*}

==> tables/so.tex <==
\begin{table}[h]
\centering
\footnotesize
\caption{Summarization of So Libraries in App Samples}
% \begin{tabular}{p{10pt}p{50pt}p{40pt}p{20pt}p{50pt}p{40pt}p{20pt}p{30pt}p{30pt}p{10pt}p{30pt}p{30pt}p{10pt}}
\begin{tabular}{lcccc}
\toprule
& \multicolumn{2}{c}{Top 20 Native Library in \target{}} & \multicolumn{2}{c}{Top 20 Native Library in \normal{} Apps}
\cr \cmidrule(lr){2-3}\cmidrule(lr){4-5} 
Rank & Name           & Rate (\%)           & Name         & Rate (\%) \cr
\midrule
1 & libpl\_droidsonroids\_gif & 46.0 & libmain & 29.2 \\
2 & lib39285EFA & 28.7 & libunity & 29.2 \\
3 & libso & 27.4 & libmono & 26.6 \\
4 & libimagepipeline & 22.0 & libmonodroid & 9.2 \\
5 & libc++\_shared & 20.6 & libmonosgen-2.0 & 9.1 \\
6 & libmsc & 17.0 & libmono-btls-shared & 6.3 \\
7 & libnative-filters & 14.2 & libCore & 6.1 \\
8 & libnative-imagetranscoder & 13.9 & libysshared & 6.1 \\
9 & libBugly & 13.8 & libgpg & 6.0 \\
10 & libRSSupport & 13.1 & libstlport\_shared & 5.9 \\
11 & librsjni & 13.1 & libimagepipeline & 5.8 \\
12 & librsjni\_androidx & 11.2 & libc++\_shared & 4.7 \\
13 & libijkplayer & 10.7 & libgifimage & 4.4 \\
14 & libijkffmpeg & 10.7 & libopenal & 3.5 \\
15 & libijksdl & 10.7 & libaacdecoder & 3.5 \\
16 & libgifimage & 10.4 & libgdx & 3.3 \\
17 & libne\_audio & 8.4 & libpl\_droidsonroids\_gif & 3.1 \\
18 & libfb & 8.2 & libstagefright\_honeycomb & 2.8 \\
19 & libyoga & 8.2 & libstagefright\_froyo & 2.8 \\
20 & libglog\_init & 8.0 & libkroll-v8 & 2.5 \\
\bottomrule
\end{tabular}
\label{tab:so}
\end{table}
